Adjacent-category models for ordinal time series and their application to climate-dependent spruce budworm defoliation dynamics

This work proposes an adjacent-category autoregressive model for time series of ordinal variables. We apply this model to dendrochronological records to study the effect of climate on the intensity of spruce budworm defoliation during outbreaks in two sites in eastern Canada. The model's parameters are estimated using the maximum likelihood approach. We show that this estimator is consistent and asymptotically Gaussian distributed. We also propose a Portemanteau test for goodness-of-fit. Our study shows that the seasonal ranges of maximum daily temperatures in the spring and summer have a significant quadratic effect on defoliation. The study reveals that for both regions, a greater range of summer daily maximum temperatures is associated with lower levels of defoliation up to a threshold estimated at 22.7C (CI of 0-39.7C at 95%) in T\'emiscamingue and 21.8C (CI of 0-54.2C at 95%) for Matawinie. For Matawinie, a greater range in spring daily maximum temperatures increased defoliation, up to a threshold of 32.5C (CI of 0-80.0C). We also present a statistical test to compare the autoregressive parameter values between different fits of the model, which allows us to detect changes in the defoliation dynamics between the study sites in terms of their respective autoregression structures.

==> source.tex <==
%\documentclass[aos,preprint]{imsart}
\usepackage[margin=1in]{geometry}% <--- 1 in margin
\RequirePackage[T1]{fontenc}
\usepackage{setspace}
\doublespacing
\RequirePackage{amsthm,amsmath}
\usepackage[round]{natbib}
\bibliographystyle{apalike}
\usepackage[english]{babel}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
%\usepackage{pgf,tikz}\usepackage{mathrsfs}\usetikzlibrary{arrows}\pagestyle{empty}
\usepackage{enumerate}
\usepackage{caption}
%\usepackage{hyperref} 
\usepackage[english]{babel}
\usepackage{nameref}
\usepackage{prepub}
\usepackage{xcolor}
\usepackage[bbgreekl]{mathbbol}
\usepackage{comment}
\usepackage{amsmath,amsfonts,amssymb,euscript,mathrsfs,mathtools, mathdots}
\usepackage{graphicx}
\usepackage[inline]{enumitem}
\usepackage[Sonny]{fncychap}
\usepackage{bigints}
\usepackage{xcolor}
%\usepackage{float}
%\usepackage[final]{pdfpages}
%\usepackage{natbib}
%\usepackage[textwidth=3cm, textsize=footnotesize]{todonotes} %%%%new command for comments
%Please add the following packages if necessary:
\usepackage{booktabs, multirow} % for borders and merged ranges
\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
\usepackage{changepage,threeparttable} % for wide tables
%\renewcommand{\baselinestretch}{1.50}


%\usepackage[latin1]{inputenc}
%\usepackage{txfonts}
%\usepackage[T1]{fontenc}
%\usepackage{slashbox}
\usepackage{fullpage}
\usepackage{algorithm}
\usepackage{algpseudocode}
%\usepackage{comment}
%\usepackage{theorem}
%\usepackage{float}
%\usepackage{setspace}
%\usepackage{latexsym}
\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{graphicx}
%\usepackage{microtype}
\usepackage{dsfont}
%\startlocaldefs
\makeatletter
\def\captionof#1#2{{\def\@captype{#1}#2}}
\makeatother
\def\1{\mbox{\bf 1}}
\def\R{\mathbb{R}}
\def\vE{\mathcal{E}}
\def\B{\mathbb{B}}
\def\N{\mathbb{N}}
\def\P{\mathbb{P}}
\def\E{\mathbb{E}}
\def\L{\mathbb{L}}
\def\F{\mathbb{F}}
\def\R{\mathbb{R}}
\def\C{\mathbb{C}}
\def\Z{\mathbb{Z}}
\def\e{\mathrm{e}}
\def\G{\mathbb{G}}
\def\D{\mathbb{D}}
\def\H{\mathbb{H}}
\def\Q{\mathbb{Q}}
\def\vec{\mathrm{vec}}
\def\v{\mbox{Var\,}}
\def\lip{\mbox{Lip\,\,}}
\def\Lip{\mbox{Lip\,\,}}
\def\c{\mbox{Cov}}
\def\co{\mbox{Corr}}
\def\dim{\mbox{dim}}\def\card{\mbox{card}}
\def\X{\mathbb{X}}
\def\yt{(Y_t = (Y_{1,t}, \ldots, Y_{p,t}))_{t \in \Z}}
\def\zt{(Z_t)_{t \in \Z}}
\def\ylx{(Y_t, \lambda_t, X_t)_{t \in \Z}}
\def\lt{(\lambda_t)_{t \in \Z}}

\newcommand{\todo}[2][red]{\textcolor{#1}{#2}}

\newcommand{\dpartial}[2]{
 \frac{\partial {#1}}{\partial {#2}}
}

\newcommand{\emphref}[1]{
\emph{\ref{#1}}
}

\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

\newcommand{\wideg}[2][1.5]{
  \mathrel{\overset{#2}{\scalebox{#1}[1]{$=$}}}
}

\newcommand{\ddpartial}[3]{
 \frac{\partial^2 {#1}}{\partial {#2} \partial {#3}}
}


\newtheorem{theo}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{Def}{Definition}
\newtheorem{cor}{Corollary}
\newtheorem{Def/Prop}{Definition-Proposition}
\newtheorem{Remark}{Remark}

\newcounter{ex}

\setcounter{ex}{1}

\renewcommand{\theex}{\thesection.\arabic{ex}}

\newenvironment{example}[1]{\begin{paragraph} {\bfseries Example \theex\ [#1] }}{\addtocounter{ex}{1}\end{paragraph}}

%\newcommand{\kostas}[1]{\todo[inline, color=yellow!20]{{\bf Kostas:} #1}}


\newcounter{exos}
\renewcommand\theexos{\arabic{exos}}
\newenvironment{exos}
{\par\refstepcounter{exos}\medskip\noindent\textsc{Exercise \theexos}\space}
{\par}
\newcounter{prob}
\renewcommand\theprob{\arabic{prob}}
\newenvironment{prob}
{\par\refstepcounter{prob}\medskip\noindent\textsc{Problème \theprob}\space}
{\par}

\newcommand{\tens}[1]{%
  \mathbin{\mathop{\otimes}\limits_{#1}}%
}


\newcounter{note}
\setcounter{note}{1}
\renewcommand{\thenote}{\thesection.\arabic{note}}
\newenvironment{notes}[1]{\begin{paragraph} {\bfseries Notes \thenote\ #1 }}{\addtocounter{note}{1}\end{paragraph}}

\makeatletter
\let\orgdescriptionlabel\descriptionlabel
\renewcommand*{\descriptionlabel}[1]{%
  \let\orglabel\label
  \let\label\@gobble
  \phantomsection
  \edef\@currentlabel{#1}%
  %\edef\@currentlabelname{#1}%
  \let\label\orglabel
  \orgdescriptionlabel{#1}%
}
\makeatother
